Sticky Brownian Rounding and its Applications to Constraint Satisfaction Problems

Semidefinite programming is a powerful tool in the design and analysis of approximation algorithms for combinatorial optimization problems. In particular, the random hyperplane rounding method of Goemans and Williamson has been extensively studied for more than two decades, resulting in various extensions to the original technique and beautiful algorithms for a wide range of applications. Despite the fact that this approach yields tight approximation guarantees for some problems, e.g., Max-Cut, for many others, e.g., Max-SAT and Max-DiCut, the tight approximation ratio is still unknown. One of the main reasons for this is the fact that very few techniques for rounding semidefinite relaxations are known. In this work, we present a new general and simple method for rounding semi-definite programs, based on Brownian motion. Our approach is inspired by recent results in algorithmic discrepancy theory. We develop and present tools for analyzing our new rounding algorithms, utilizing mathematical machinery from the theory of Brownian motion, complex analysis, and partial differential equations. Focusing on constraint satisfaction problems, we apply our method to several classical problems, including Max-Cut, Max-2SAT, and MaxDiCut, and derive new algorithms that are competitive with the best known results. To illustrate the versatility and general applicability of our approach, we give new approximation algorithms for the Max-Cut problem with side constraints that crucially utilizes measure concentration results for the Sticky Brownian Motion, a feature missing from hyperplane rounding and its generalizations

==> numerical_experiments.tex <==
In this section we describe how we obtain the approximation factors of the introduced rounding algorithms, numerically. 
First, let us define what a \textit{configuration} is. 
Let $\bv_0,\bv_1,\ldots, \bv_n$ be the solution vectors of the SDP relaxation.
Each subset of size $d$ of these vectors forms a $d$-dimensional spatial configuration.
Based on the problem that we want to solve, we are only interested in particular values of $d$. For example, in all of the binary Max-2-CSP problems that we consider, we are interested in 3-dimensional configurations consisting of $\bv_0$ and two other vectors.

The idea is that for a given configuration, we can find its contribution in the SDP relaxation (based on the objective of the relaxation).
Moreover, we are able to compute the expected value of the rounding procedure.
Thus, we determine the expected approximation ratio of the rounding for this specific configuration. 
By repeating this procedure on all of the feasible configurations for a problem of interest (e.g., \MC), and taking their minimum, we will find the expected approximation factor of the rounding algorithm on this problem for all instances.

In order to enumerate all the configurations, we need to discretize the space of possible configurations.
The discretization can be done based on the representation that we choose for $\bv_i$. 
As defined in the preliminaries section, we can write each vector $\bv_i$ as $\bv_i = x_i\bv_0+\bw_i$. 
Based on this notation, each two vectors $\bv_i$ and $\bv_j$ can be realized by having $x_i$ and $x_j$ and also the angle between vectors $\bw_i$ and $\bw_j$, denoted by $\theta_{ij}$. 
In other words, each configuration is of the form $conf_{ij} = (x_i, x_j, \theta_{ij})$, where $x_i,x_j \in [0,1]$ and $\theta_{ij} \in [0, \pi]$. 
Note that $conf_{i,j}$ implicitly considers $\bv_0$ as well.
The whole process of finding the approximation factor of a given problem is described in Algorithm~\ref{alg:discretized-apx-finder}. 
In what follows, $obj_C(x_i,x_j, \theta_{ij})$ is equivalent with $p_C(x)$ as defined in the preliminaries with a slight change that $obj_C(x_i,x_j, \theta_{ij})$ explicitly states the objective of clause $C$ in terms of its inputs (instead of $x_i, x_j$ and $x_{ij}$).
\begin{algorithm}
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{$obj_C(x_i,x_j,\theta_{ij})$, and discretization level $0<\delta<1$.}
\KwOut{Approximation factor of the rounding for problem $\mathcal{P}$.}
Let $S = \{k\delta | 0\leq k \leq 1/\delta\}$ and $R=\{k\delta | 0\leq k \leq \pi/\delta\}$\;
$apx=1$\;
\ForAll{$conf_{ij} \in S\times S \times R$} {
  \If{$conf_{ij}$ satisfies the triangle inequalities} {
    $sdp\_val_{ij} = obj_C(conf_{ij})$\;
    $round_{ij} = $ \sc{Get-Rounding-Value($conf_{ij}$)}\;
    \If{$round_{ij} / sdp\_val_{ij} < apx$}{
        $apx = round_{ij} / sdp\_val_{ij}$\;
    }
  }
}
\Return{$apx$}\;
\caption{Discretized Approximation Finder for binary 2-CSP problem $\mathcal{P}$}
\label{alg:discretized-apx-finder}
\end{algorithm}
\saznote{{\sc{Get-Rounding-Value}} subroutine should be added based on the PDE's.}

Algorithm~\ref{alg:discretized-apx-finder} discards all the configurations which violate the triangle inequalities as they cannot be appeared in the solution of the SDP.
Further, it uses subroutine {\sc{Get-Rounding-Value($conf_{ij}$)}} that returns the expected value of the rounding algorithm for $conf_{ij}$.
This value can be computed (in expectation) using two different approaches:
\begin{enumerate}
    \item Directly simulating the algorithm's diffusion process and repeating it sufficiently many times to obtain the expected value of the rounding with high probability.
    \item Numerically solving the corresponding boundary value PDE of the process which is also equivalent to the expected rounded value.
\end{enumerate}
We implemented both of these approaches for the basic walk, and as we expected, we observed that the results of these two approaches are consistent.
Nonetheless, in all of the reported results, we employed the PDE approach for computing {\sc{Get-Rounding-Value($conf_{ij}$)}} (unless stated otherwise).
Note that from the practical point of view, it is straightforward to extend this framework to higher dimensional configurations as long as we have enough computational power.
Now we are ready to present the observations for specific problems.

\subsection{\MC}
In order to use Algorithm~\ref{alg:discretized-apx-finder}, the objective function of the \MC problem for a given clause $C$ can be written as follows:
\begin{equation*}
    obj_C(conf_{ij}) = x_i+x_j-2x_ix_j-2\sqrt{(x_i-x_i^2)(x_j-x_j^2)}\cos{\theta}.
\end{equation*}
Also, the discretization level $\delta$ is set to be $0.02$.
The basic, slowdown, and exponential PDE's are as defined before for 2-CSP problems, and the boundary value function for \MC is as follows:
\begin{equation*}
    b(x,y) = x+y-2xy, \forall (x,y) \in \partial [0,1]^2.
\end{equation*}

By fixing the values $x_i$ and $x_j$ and varying $\theta_{ij}$, we can get a better intuition of the behavior of the rounding algorithm.
For this purpose, Figure~\ref{fig:maxcut-configurations} illustrates the probability of cutting an edge for the basic walk for two configurations $(0.4, 0.4, \theta_{ij})$ and $(0.4, 0.6, \theta_{ij})$. 
These figures contain the baseline probability $\theta_{ij}/\pi$ as it obtains the optimal approximation ratio (under Unique Games Conjecture).
Furthermore, it can be verified that when $\theta_{ij} \leq \pi/2$, the process always returns a better result than the SDP relaxation value.
We also observe that for some angles the triangle inequalities are not satisfied.
\begin{figure}[ht]
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/maxcut-basic-0404.png}
  \caption{$conf_{ij}=(0.4,0.4,\theta_{ij})$}
\end{subfigure}%
\hspace{0.02\textwidth}
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/maxcut-basic-0406.png}
  \caption{$conf_{ij}=(0.4,0.6,\theta_{ij})$}
\end{subfigure}
\caption{Comparing the probability of cutting an edge of the basic walk with the SDP value and also the optimal probability of $\theta/\pi$ (i.e., baseline) for two different set of configurations.}
\label{fig:maxcut-configurations}
\end{figure}

Note that none of the configurations in Figure~\ref{fig:maxcut-configurations} are of interest for the \MC problem. 
The reason, as stated before, is that we can always assume that any configuration can be transformed to a configuration with all the marginals set to half without any loss in the value.
Therefore, in order to find the worst-case result, it is enough to find the minimum ratio for configuration $(0.5, 0.5, \theta_{ij})$. 
Table~\ref{tab:max-cut-ratios} shows these minimum ratios which in fact reflects the achieved approximation ratio for basic walk, slowdown walk, and also exponential walk. 
Also, Figure~\ref{fig:maxcut-worst-case} depicts the performance for these walks on the mentioned configuration.
This figure shows the observed progress in the approximation ratio by changing the walk from basic to exponential.
Due to the guaranteed error of the numerical solver, we cannot report higher precision values, however, we conjecture that exponential walk performs equally as the optimal random hyperplane rounding. 

\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
         \hline
         Process Type & Approximation Ratio\\
         \hline
         Basic & $0.85$  \\
         Slowdown & $0.86$\\
         Exponential & $0.87$\\
         \hline
    \end{tabular}
    \caption{Approximation ratio of basic, slowdown, and exponential walks for the \MC problem.}
    \label{tab:max-cut-ratios} 
\end{table}

\begin{figure}[ht]
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/maxcut-basic-0505.png}
  \caption{Basic walk}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/maxcut-slow-0505.png}
  \caption{Slowdown walk}
\end{subfigure}%
\hspace{0.01\textwidth}
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/maxcut-exp161-0505.png}
  \caption{Exponential walk}
\end{subfigure}
\caption{Comparing the performance of three walks on $conf_{ij}=(0.5,0.5,\theta_{ij})$.}
\label{fig:maxcut-worst-case}
\end{figure}

\subsection{\MtwoSAT}
We use the following objective function for the \MtwoSAT problem:
\begin{equation*}
    obj_C(conf_{ij}) = x_i + x_j - x_ix_j - \sqrt{(x_i-x_i^2)(x_j-x_j^2)}\cos{\theta}.
\end{equation*}
Like the previous experiment, the discretization level $\delta$ is $0.02$.
Also, the boundary value is as follows:
\begin{equation*}
    b(x,y) = \min\big\{1, \max\{x,y\}\big\}, \forall (x,y) \in \partial [0,1]^2.
\end{equation*}
Unlike \MC, we no longer can limit the configurations to the all-half marginals.
Therefore, in order to find the worst-case approximation, we explore all the feasible configurations. 
By doing so for all three different walks, we obtain the approximation ratios reported in Table~\ref{tab:max2sat-approximation}.
\saznote{I should change the numbers of this table after rerunning the experiments.}
\begin{table}[ht]
    \centering
    \begin{tabular}{|c|c|c|}
         \hline
         Process Type & Approximation Ratio\\
         \hline
         Basic & $0.921$  \\
         Slowdown & $0.927$\\
         Exponential & $0.927$\\
         \hline
    \end{tabular}
    \caption{Approximation ratio of basic, slowdown, and exponential walks for the \MtwoSAT problem.}
    \label{tab:max2sat-approximation} 
\end{table}

Comparing slowdown and exponential walks, we observe that although the behavior of the algorithm slightly changes, the worst-case happens at exactly the same configurations which results in the same approximation ratios.
The performance of these walks has been plotted in Figure~\ref{fig:max2sat-worst-case} by fixing $x_i$ and $x_j$ of the worst-case configuration.
Since the difference between slowdown and exponential walks could not be even distinguished on the same plot, we have only included one of them.
\begin{figure}[ht]
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/max2sat-basic-worst38-40.png}
  \caption{Basic walk; $conf_{ij}=(0.38,0.40,\theta_{ij})$}
\end{subfigure}%
\hspace{0.02\textwidth}
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{Figures/max2sat-exp161-worst36-38.png}
  \caption{Exponential walk; $conf_{ij}=(0.36,0.38,\theta_{ij})$}
\end{subfigure}%
\caption{Comparing the performance of basic walk and exponential walk for the \MtwoSAT problem.}
\label{fig:max2sat-worst-case}
\end{figure}


==> preliminaries.tex <==
Guru changes this.

\rsnote{bla bla bla... again :-)}

\subsection{SDP Formulation}
Recall that a binary Max-$2$-CSP problem is defined by a collection of
predicates $\Pi$, where each $p \in \Pi$ is a boolean function on
$\{0,1\}^2$. An instance of the problem is collection of clauses $\CC
\subseteq {[n] \choose 2}$, where each $C \in \CC$ has an associated
weight $a_C \ge 0$ and a predicate $p_C$ from $\Pi$. Suppose $x \in
\{0,1\}^n$ is some assignment of values to each variable $i$. We abuse
notation slightly and write $p_C(x)$ for $p_C(x_i, x_j)$ where $C =
\{x_i, x_j\}$.  The objective of the problem is to find an assignment
$x$ so that the weight of satisfied clauses given by $\sum_{C: p_C(x)
  = 1} a_C$ is maximized.

We use the following SDP relaxation of a Max-$2$-CSP problem:
\begin{align}
  &\text{Maximize}
  \sum_{C \in \CC}a_C(\widehat{p}_C(0) + \widehat{p}_C(i)x_i +
  \widehat{p}_C(j)x_j + \widehat{p}_C(i,j)x_{ij}) \label{eq:genSDP-obj}\\
  \text{s.t.}~\\
  &x_{ii} = x_i \ \ \ \forall i \in \{1, \ldots, n\}\\
  &x_{ij} \ge 0 \ \ \ \forall i, j \in \{1, \ldots, n\}\label{eq:genSDP-SA1}\\
  &\min\{x_i, x_j\} \ge x_{ij} \ \ \ \forall i, j \in \{1, \ldots,  n\}\label{eq:genSDP-SA2}\\
  &1 - x_i - x_j + x_{ij} \ge 0 \ \ \ \forall i, j \in \{1, \ldots, n\}\label{eq:genSDP-SA3}\\
  &X \succeq 0.\label{eq:genSDP-psd}
\end{align}
Above, $\widehat{p}_C(0), \widehat{p}_C(i), \widehat{p}_C(j),
\widehat{p}_C(i,j)$ are the unique reals for which
\[
p_C(x) =
\widehat{p}_C(0) + \widehat{p}_C(i)x_i + \widehat{p}_C(j)x_j + \widehat{p}_C(i,j)x_ix_j
\]
for every $x \in \{0,1\}^n$. The matrix $X$ in \eqref{eq:genSDP-psd}
is indexed by $\{0, \ldots, n\}$ and is given by
\[
X =
\begin{pmatrix}
  1 & x_1 & \cdots & x_n\\
  x_1 & x_{11} & \cdots & x_{1n} \\
  \vdots & \vdots & \ddots & \vdots\\
  x_n & x_{n1} & \cdots & x_{nn}\\
\end{pmatrix}.
\]
This relaxation is equivalent to the one used by
Raghavendra~\cite{Raghavendra08}, who showed that, assuming the Unique
Games conjecture, it achieves optimal approximation for any Max-CSP.

We focus on two examples of Max-$2$-CSPs: Max-Cut and Max-$2$-Sat. For
Max-Cut we will think of the instance as an undirected graph $G =
([n], E)$ with edge weights $a_e$. For Max-$2$-Sat we use the
Max-$2$-CSP notation introduced above. However, to simplify notation,
we introduce variables $x_{-1}, \ldots, x_{-n}$ with the constraint
$x_{-i} = 1 - x_i$. I.e.~$x_{-i}$ is the negation of $x_i$. This way, we
can write all clauses of the Max-2-Sat instance over
this extended set of variables without negations.

The general SDP relaxation~\cref{eq:genSDP-obj,eq:genSDP-psd} %\eqref{eq:genSDP-obj}--\eqref{eq:genSDP-psd}
specializes to the following relaxations: %for these two problems.
\begin{center}
  \begin{tabular}[h]{|p{0.4\linewidth}|p{0.6\linewidth}|} \hline
    { \textbf{Max-Cut}
      \begin{align}
        &\text{Maximize} \sum_{(i,j) \in E}{a_{ij}(1 - 2x_{ij})}\label{eq:Cut-obj}\\
        &\text{s.t.}~\\
        &x_{ii} = x_i = \frac12 \ \ \ \forall i \in \{1, \ldots, n\}\\
        &x_{ij} \ge 0 \ \ \ \forall i, j \in \{1, \ldots, n\}\\
        &X \succeq 0.\label{eq:Cut-psd}
      \end{align}
    }&
    { \textbf{Max-$2$-Sat}
      \begin{align}
        &\text{Maximize}
        \sum_{C \in \CC}a_C(1 - x_{ij}) \label{eq:2Sat-obj}\\
        &\text{s.t.}~\\
        &x_{-i} = 1-x_i \ \ \ \forall i \in \{1, \ldots, n\}\\
        &x_{-i,j} = x_j - x_{ij}\ \ \ \forall i, j \in \{-n, \ldots,
        n\}\setminus \{0\}\\
        &x_{ii} = x_i \ \ \ \forall i \in \{-n, \ldots, n\}\setminus \{0\}\\
        &x_{ij} \ge 0 \ \ \ \forall i, j \in \{-n, \ldots, n\}\setminus \{0\}\\
        &\min\{x_i, x_j\} \ge x_{ij} \ \ \ \forall i, j \in \{-n, \ldots,  n\}\setminus \{0\}\\
        &1 - x_i - x_j + x_{ij} \ge 0 \ \ \ \forall i, j \in \{-n, \ldots,n\}\setminus \{0\}\\
        &X \succeq 0.\label{eq:2Sat-psd}
      \end{align}
    }\\
    \hline
  \end{tabular}
\end{center}
Note that simply following
\eqref{eq:genSDP-obj}--\eqref{eq:genSDP-psd} would give the objective
$x_i + x_j - 2x_{ij}$ and arbitrary values for $x_i$ and $x_j$ in the
case of Max-Cut. However, since both the objective and the constraints
are symmetric under the substitution of $x_i$ with $1-x_i$ and $x_{ij}$ with $1
- x_i - x_j + x_{ij}$, the SDP always has an optimal
solution in which $x_i = \frac12$ for all $i \in [n]$.

When designing rounding algorithms, it is convenient to work with the
Cholesky factorization of the PSD matrix $X$ given by a solution to
\eqref{eq:genSDP-obj}--\eqref{eq:genSDP-psd}. We write $X = V^\top V$,
and denote the columns of the matrix $V$ by $v_0, \ldots, v_n$. Then,
$x_{ij} = v_i^\top v_j$ and $x_i = v_0^\top v_i$.

The constraints of the SDP imply that
\begin{align*}
  \|v_0\|^2 &= 1,
  &\|v_i\|^2= v_0^\top v_i = x_i.
\end{align*}
Equivalently, each vector $v_i$ lies on the Euclidean sphere with
radius $\frac12$ centered at $\frac12 v_0$.

It will also be convenient to consider separately the component of
each vector $v_i$ in the direction of $v_0$, and the component
orthogonal to $v_0$. We write $w_i = v_i - x_i v_0$ for this latter
component. The length of $w_i$ is given by $\|w_i\|^2 = x_i - x_i^2$.

\textbf{Triangle Inequalities:} Using
the equality $x_{ij} = x_i x_j + w_i^\top w_j$, the
constraints \eqref{eq:genSDP-SA1}--\eqref{eq:genSDP-SA3} imply the
following inequalities:
\begin{align*}
  w_i^\top w_j &\ge -x_i x_j\\
  w_i^\top w_j &\ge -(1-x_i)(1- x_j)\\
  w_i^\top w_j &\le \min\{x_i(1-x_j), (1-x_i)x_j\}.
\end{align*}
In the case when $w_i, w_j \neq 0$, we denote the angle between $w_i$
and $w_j$ by $\theta_{ij}$, and we write $\widehat{w}_i =
\frac{w_i}{\|w_i\|}$ for the unit vector in the direction of $w_i$,
and analogously for $w_j$. Then $\cos \theta_{ij} = \widehat{w}_i^\top
\widehat{w}_j$ satisfies the inequalities
\begin{equation*}
  -\min\left\{\alpha, \frac1\alpha\right\} \le
  \cos \theta_{ij}
  \le
  \min\left\{\beta, \frac1\beta\right\},
\end{equation*}
where $\alpha = \sqrt{\frac{x_i x_j}{(1-x_i)(1-x_j)}}$ and
$\beta = \sqrt{\frac{x_i(1-x_j)}{(1-x_i)x_j}}$.



